Efficient Activation Function Optimization through Surrogate Modeling

Carefully designed activation functions can improve the performance of neural networks in many machine learning tasks. However, it is difficult for humans to construct optimal activation functions, and current activation function search algorithms are prohibitively expensive. This paper aims to improve the state of the art through three steps: First, the benchmark datasets Act-Bench-CNN, Act-Bench-ResNet, and Act-Bench-ViT were created by training convolutional, residual, and vision transformer architectures from scratch with 2,913 systematically generated activation functions. Second, a characterization of the benchmark space was developed, leading to a new surrogate-based method for optimization. More specifically, the spectrum of the Fisher information matrix associated with the model's predictive distribution at initialization and the activation function's output distribution were found to be highly predictive of performance. Third, the surrogate was used to discover improved activation functions in several real-world tasks, with a surprising finding: a sigmoidal design that outperformed all other activation functions was discovered, challenging the status quo of always using rectifier nonlinearities in deep learning. Each of these steps is a contribution in its own right; together they serve as a practical and theoretical foundation for further research on activation function optimization.

==> figures/training_details.tex <==
% \newcommand\tabwidthmul{1.0}

% \begin{table*}
%     \centering
%     \caption{Training details and hyperparameter values used in the experiments.\\}
%     \adjustbox{max width=\tabwidthmul\linewidth}{%
%     \begin{tabular}{ll}
%         \toprule
%         \multicolumn{2}{c}{All-CNN-C on CIFAR-10 and CIFAR-100} \\
%         \midrule
%         Batch Size & 128 \\
%         Dropout & 0.5 \\
%         Epochs & 25 for \texttt{Act-Bench-CNN} and search (Figure \ref{fig:search_progress}), 50 for full evaluation (Table \ref{tab:search_results}) \\
%         Image Size & $32 \times 32$ \\
%         Learning Rate & Linear warmup to 0.1 for five epochs, then linear decay \\
%         Mean/Std. Normalization & Yes \\
%         Momentum & 0.9 \\
%         Optimizer & SGD \\
%         Random Crops & $ 32 \times 32$ crops of images padded with four pixels on all sides \\
%         Random Flips & Yes \\
%         Weight Decay & $1e^{-4}$ \\
%         Weight Initialization & AutoInit \cite{bingham2021autoinit} \\
%         \bottomrule
%     \end{tabular}
%     }\\
%     \vspace{1em}

%     \adjustbox{max width=\tabwidthmul\linewidth}{%
%     \begin{tabular}{ll}
%         \toprule
%         \multicolumn{2}{c}{ResNet-56 on CIFAR-10 and CIFAR-100} \\
%         \midrule
%         Batch Size & 128 \\
%         Dropout & 0.0 \\
%         Epochs & 25 for \texttt{Act-Bench-ResNet} and search (Figure \ref{fig:search_progress}), 50 for full evaluation (Table \ref{tab:search_results}) \\
%         Image Size & $32 \times 32$ \\
%         Learning Rate & Linear warmup to 0.1 for five epochs, then linear decay \\
%         Mean/Std. Normalization & No \\
%         Momentum & 0.9 \\
%         Optimizer & SGD \\
%         Random Crops & $ 32 \times 32$ crops of images padded with five pixels on all sides \\
%         Random Flips & Yes \\
%         Weight Decay & $1e^{-4}$ \\
%         Weight Initialization & AutoInit \cite{bingham2021autoinit} \\
%         \bottomrule
%     \end{tabular}
%     }\\
%     \vspace{1em}

%     \adjustbox{max width=\tabwidthmul\linewidth}{%
%     \begin{tabular}{ll}
%         \toprule
%         \multicolumn{2}{c}{MobileViTv2-0.5 on Imagenette and ImageNet} \\
%         \midrule
%         Batch Size & 256 \\
%         CutMix Alpha \cite{yun2019cutmix} & 1.0 \\
%         Epochs & 105 \\
%         Evaluation Center Crop & 95\% \\
%         Image Size & $160 \times 160$ \\
%         Learning Rate & Linear warmup from $1e^{-4}$ to $4e^{-3}$ for five epochs, then cosine decay to $1e^{-6}$\\
%         Mixup Alpha \cite{zhang2017mixup} & 0.1 \\
%         Optimizer & AdamW \cite{loshchilov2017decoupled} \\
%         RandAugment \cite{cubuk2020randaugment} & Magnitude six, applied twice \\
%         Random Resized Crop \cite{szegedy2015going} & Minimum 8\% of the original image \\
%         Weight Decay & $0.02\times$ current learning rate \\
%         \bottomrule
%     \end{tabular}
%     }\\
%     \vspace{1em}

%     \adjustbox{max width=\tabwidthmul\linewidth}{%
%     \begin{tabular}{ll}
%         \toprule
%         \multicolumn{2}{c}{ResNet-50 on ImageNet} \\
%         \midrule
%         Batch Size & 256 \\
%         CutMix Alpha \cite{yun2019cutmix} & 1.0 \\
%         Epochs & 105 \\
%         Evaluation Center Crop & 95\% \\
%         Image Size & $160 \times 160$ \\
%         Learning Rate & Linear warmup from $1e^{-4}$ to $2e^{-3}$ for five epochs, then cosine decay to $1e^{-6}$\\
%         Mixup Alpha \cite{zhang2017mixup} & 0.1 \\
%         Optimizer & AdamW \cite{loshchilov2017decoupled} \\
%         RandAugment \cite{cubuk2020randaugment} & Magnitude six, applied twice \\
%         Random Resized Crop \cite{szegedy2015going} & Minimum 8\% of the original image \\
%         Weight Decay & $0.02\times$ current learning rate \\
%         Weight Initialization & AutoInit \cite{bingham2021autoinit} \\
%         \bottomrule
%     \end{tabular}
%     }

%     \label{tab:training_details}
% \end{table*}

